Blended Diffusion for Text-driven Editing of Natural Images

Natural language offers a highly intuitive interface for image editing. In this paper, we introduce the first solution for performing local (region-based) edits in generic natural images, based on a natural language description along with an ROI mask. We achieve our goal by leveraging and combining a pretrained language-image model (CLIP), to steer the edit towards a user-provided text prompt, with a denoising diffusion probabilistic model (DDPM) to generate natural-looking results. To seamlessly fuse the edited region with the unchanged parts of the image, we spatially blend noised versions of the input image with the local text-guided diffusion latent at a progression of noise levels. In addition, we show that adding augmentations to the diffusion process mitigates adversarial results. We compare against several baselines and related methods, both qualitatively and quantitatively, and show that our method outperforms these solutions in terms of overall realism, ability to preserve the background and matching the text. Finally, we show several text-driven editing applications, including adding a new object to an image, removing/replacing/altering existing objects, background replacement, and image extrapolation. Code is available at: https://omriavrahami.com/blended-diffusion-page/

==> document.tex <==
The forward noising process effectively defines a sequence of image manifolds, where the images become progressively more noisy. The reverse, denoising diffusion process, in each stage projects a noisy image onto the next, less noisy, manifold.
To create a seamless result where one region complies with a guiding prompt, while the rest is identical to the original input image, we spatially blend the noisy images progressively generated by the CLIP-guided process with all the noisy versions of the input image. While, in each step along the way, the result of the blending is not guaranteed to be coherent, the denoising diffusion step that follows restores coherence by projecting onto the next manifold. 
